A higher order nonconforming virtual element method for the Cahn-Hilliard equation

In this paper we develop a fully nonconforming virtual element method (VEM) of arbitrary approximation order for the two dimensional Cahn-Hilliard equation. We carry out the error analysis for the semidiscrete (continuous-in-time) scheme and verify the theoretical convergence result via numerical experiments. We present a fully discrete scheme which uses a convex splitting Runge-Kutta method to discretize in the temporal variable alongside the virtual element spatial discretization.

==> Results/FiguresRevised/evolutionScreenshots.tex <==
% \ifthenelse{\boolean{thesis}}{
    \begin{figure}[p]
        % \centering
            \begin{center}
                \subfloat[Evolution of a cross at time $t=0$ with order $\polOrder=4$ on the $N=25$ grids.]{\label{fig: evolution time t=0}
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_criss_epsFac25_p4_N25_dt10_polygons.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac25_p4_N25_dt10_polygons.png}
                }
                \subfloat[]{
                % \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_criss_epsFac100_p4_N25_dt10_polygons.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac100_p4_N25_dt10_polygons.png}} 
            \end{center}
            \begin{center}
                \subfloat[Evolution of a cross at time $t=0.004$.]
                % for the polynomial order $\polOrder=4$ on the $25 \times 25$ grids.]
                {\label{fig: evolution time t=0.004}
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_criss_epsFac25_p4_N25_dt10_00001.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac25_p4_N25_dt10_00001.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_criss_epsFac100_p4_N25_dt10_00001.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac100_p4_N25_dt10_00001.png}}
            \end{center}
            \begin{center}
                \subfloat[Evolution of a cross at time $t=0.8$.]
                % for the polynomial order $\polOrder=4$ on the $25 \times 25$ grids.]
                {\label{fig: evolution at time t=0.8}
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_criss_epsFac25_p4_N25_dt10_00199.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac25_p4_N25_dt10_00199.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_criss_epsFac100_p4_N25_dt10_00199.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac100_p4_N25_dt10_00199.png}}
            \end{center}
        \caption{Test 2: evolution of a cross for order $\polOrder=4$ on the $N=25$ grids displayed at three different time frames from top to bottom $(t=0,0.004,0.8)$. The first two columns correspond to $\eps=1/25$ on the structured simplex mesh and the Voronoi polygonal mesh respectively. The last two columns correspond to $\eps=1/100$ on the structured simplex mesh and the Voronoi polygonal mesh respectively. }
        \label{fig: evolutionScreenshots}
    \end{figure}
% }{
    \begin{figure}[p]
        \begin{center}
            \subfloat[Evolution of a cross shaped interface with $\eps=1/100$.]{\label{fig: evolution time t=0}
            \includegraphics[width=0.25\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac100_p4_N25_dt10_polygons.png}
            \,
            \includegraphics[width=0.25\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac100_p4_N25_dt10_00001.png}
            \,
            \includegraphics[width=0.25\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac100_p4_N25_dt10_00199.png}}
        \end{center}
        \begin{center}
            \subfloat[Evolution of a cross shaped interface with $\eps=1/25$.]
            % for the polynomial order $\polOrder=4$ on the $25 \times 25$ grids.]
            {\label{fig: evolution time t=0.004}
            \includegraphics[width=0.25\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac25_p4_N25_dt10_polygons.png}
            \,
            \includegraphics[width=0.25\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac25_p4_N25_dt10_00001.png}
            \,
            \includegraphics[width=0.25\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac25_p4_N25_dt10_00199.png}}
        \end{center}
        \caption{Test 2: evolution of a cross for order $\polOrder=4$ on the $N=25$ Voronoi polygonal mesh displayed at three different time frames from left to right $(t=0,0.004,0.8)$. The first row corresponds to $\eps=1/100$ and the second row corresponds to $\eps=1/25$. }
        \label{fig: evolutionScreenshots}
    \end{figure}
% }

% \ifthenelse{\boolean{thesis}}{
    \begin{figure}[p]
        % \centering
            \begin{center}
                \subfloat[Evolution of a cross at time $t=0$ with order $\polOrder=4$ on the $N=25$ grids.]{\label{fig: evolution time t=0}
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_criss_epsFac25_p4_N25_dt10_polygons.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac25_p4_N25_dt10_polygons.png}
                }
            \end{center}
            \begin{center}
                \subfloat[Evolution of a cross at time $t=0.004$.]
                % for the polynomial order $\polOrder=4$ on the $25 \times 25$ grids.]
                {\label{fig: evolution time t=0.004}
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_criss_epsFac25_p4_N25_dt10_00001.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac25_p4_N25_dt10_00001.png}
                }
            \end{center}
            \begin{center}
                \subfloat[Evolution of a cross at time $t=0.8$.]
                % for the polynomial order $\polOrder=4$ on the $25 \times 25$ grids.]
                {\label{fig: evolution at time t=0.8}
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_criss_epsFac25_p4_N25_dt10_00199.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac25_p4_N25_dt10_00199.png}
                }
            \end{center}
        \caption{Test 2: evolution of a cross for order $\polOrder=4$ on the $N=25$ grids displayed at three different time frames from top to bottom $(t=0,0.004,0.8)$. The first two columns correspond to $\eps=1/25$ on the structured simplex mesh and the Voronoi polygonal mesh respectively. The last two columns correspond to $\eps=1/100$ on the structured simplex mesh and the Voronoi polygonal mesh respectively. }
        \label{fig: evolutionScreenshots}
    \end{figure}

    \begin{figure}[p]
        % \centering
            \begin{center}
                \subfloat[Evolution of a cross at time $t=0$ with order $\polOrder=4$ on the $N=25$ grids.]{\label{fig: evolution time t=0}
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_criss_epsFac25_p4_N25_dt10_polygons.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac25_p4_N25_dt10_polygons.png}
                }
            \end{center}
            \begin{center}
                \subfloat[Evolution of a cross at time $t=0.004$.]
                % for the polynomial order $\polOrder=4$ on the $25 \times 25$ grids.]
                {\label{fig: evolution time t=0.004}
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_criss_epsFac25_p4_N25_dt10_00001.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac25_p4_N25_dt10_00001.png}
                }
            \end{center}
            \begin{center}
                \subfloat[Evolution of a cross at time $t=0.8$.]
                % for the polynomial order $\polOrder=4$ on the $25 \times 25$ grids.]
                {\label{fig: evolution at time t=0.8}
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_criss_epsFac25_p4_N25_dt10_00199.png}
                \,
                \includegraphics[width=0.2\textwidth]{Results/FiguresRevised/chTest_crossevo_SecondOrder1_voronoi_epsFac25_p4_N25_dt10_00199.png}
                }
            \end{center}
        \caption{Test 2: evolution of a cross for order $\polOrder=4$ on the $N=25$ grids displayed at three different time frames from top to bottom $(t=0,0.004,0.8)$. The first two columns correspond to $\eps=1/25$ on the structured simplex mesh and the Voronoi polygonal mesh respectively. The last two columns correspond to $\eps=1/100$ on the structured simplex mesh and the Voronoi polygonal mesh respectively. }
        \label{fig: evolutionScreenshots}
    \end{figure}

==> Results/TablesRevised/ch_convergencespatial_FE-BE_criss_p2.tex <==
\begin{table}[h]
% \centering
\caption{Test 1: $L^2, H^1,$ and $H^2$ errors for the VEM convergence test on a structured simplex grid with polynomial order $\polOrder=2$.}
\label{tab: ch_convergencespatial_FE-BE_criss_p2}
\begin{tabular}{rrc|cc|cc|cc}
\toprule
 size &  dofs &    $h$ & $L^2$-error & $L^2$-eoc & $H^1$-error & $H^1$-eoc & $H^2$-error & $H^2$-eoc \\
\midrule
   50 &   121 & 0.2828 &  7.6681e-02 &       --- &  8.4624e-01 &       --- &  1.0749e+01 &       --- \\
  200 &   441 & 0.1414 &  1.8807e-02 &      2.03 &  2.3206e-01 &      1.87 &  5.0432e+00 &      1.09 \\
  800 &  1681 & 0.0707 &  4.7357e-03 &      1.99 &  6.0434e-02 &      1.94 &  2.4566e+00 &      1.04 \\
 3200 &  6561 & 0.0354 &  1.2908e-03 &      1.88 &  1.6157e-02 &       1.9 &  1.2193e+00 &      1.01 \\
\bottomrule
\end{tabular}
\end{table}


==> Results/TablesRevised/ch_convergencespatial_FE-BE_criss_p3.tex <==
\begin{table}[h]
\centering
\caption{Test convergencespatial with time stepping method FE-BE on a criss grid, with polynomial order p3}
\label{tab: ch_convergencespatial_FE-BE_criss_p3}
\begin{tabular}{rrc|cc|cc|cc}
\toprule
 size &  dofs &    $h$ & $L^2$-error & $L^2$-eoc & $H^1$-error & $H^1$-eoc & $H^2$-error & $H^2$-eoc \\
\midrule
   50 &   291 & 0.2828 &  8.3455e-03 &       --- &  1.0528e-01 &       --- &  2.6596e+00 &       --- \\
  200 &  1081 & 0.1414 &  5.6595e-04 &      3.88 &  1.0190e-02 &      3.37 &  6.2558e-01 &      2.09 \\
  800 &  4161 & 0.0707 &  1.8904e-04 &      1.58 &  2.0313e-03 &      2.33 &  1.4894e-01 &      2.07 \\
 3200 & 16321 & 0.0354 &  1.8130e-04 &      0.06 &  1.6269e-03 &      0.32 &  3.9364e-02 &      1.92 \\
\bottomrule
\end{tabular}
\end{table}


==> Results/TablesRevised/ch_convergencespatial_FE-BE_voronoi_p2.tex <==
\begin{table}[h]
\centering
\caption{Test 1: $L^2, H^1,$ and $H^2$ errors for the VEM convergence test on a Voronoi polygonal grid with polynomial order $\polOrder=2$.}
\label{tab: ch_convergencespatial_FE-BE_voronoi_p2}
\begin{tabular}{rrc|cc|cc|cc}
\toprule
 size &  dofs &    $h$ & $L^2$-error & $L^2$-eoc & $H^1$-error & $H^1$-eoc & $H^2$-error & $H^2$-eoc \\
\midrule
   25 &   128 & 0.3288 &  2.8739e-01 &       --- &  2.5486e+00 &       --- &  2.2657e+01 &       --- \\
  100 &   503 & 0.1535 &  7.7794e-02 &      1.72 &  7.2044e-01 &      1.77 &  8.2256e+00 &      1.62 \\
  400 &  2003 & 0.0751 &  1.0284e-02 &      2.66 &  1.0183e-01 &      2.74 &  3.1089e+00 &      1.55 \\
 1600 &  8003 & 0.0402 &  2.6221e-03 &      1.79 &  2.6065e-02 &      1.91 &  1.5340e+00 &      1.13 \\
\bottomrule
\end{tabular}
\end{table}

==> Results/TablesRevised/test1Table.tex <==
\ifthenelse{\boolean{thesis}}{}{
    \begin{table}
        \addtolength{\tabcolsep}{-0.5pt}
        {\footnotesize
            \captionsetup{position=top}
            \caption{
            Test 1: $L^2, H^1,$ and $H^2$ errors and convergence rates for the convergence test on a structured simplex grid.
            }
            \begin{center}
                \input{Results/TablesRevised/ch_convergencetemporal_FE-BE_criss_p2}
                \input{Results/TablesRevised/ch_convergencetemporal_SecondOrder1_criss_p2}
                \input{Results/TablesRevised/ch_convergencetemporal_SecondOrder1_criss_p4}
            \end{center}
        }
        \label{tab: simplex grid result}
    \end{table}
}

\ifthenelse{\boolean{thesis}}{
    \begin{table}
        \addtolength{\tabcolsep}{-0.5pt}
        {\footnotesize
            \captionsetup{position=top}
            \caption{
                Test 1: $L^2, H^1,$ and $H^2$ errors and convergence rates for the convergence test on a Voronoi polygonal grid.
                }
            \begin{center}
                \input{Results/TablesRevised/ch_convergencetemporal_FE-BE_voronoi_p2}
                \input{Results/TablesRevised/ch_convergencetemporal_SecondOrder1_voronoi_p2}
                \input{Results/TablesRevised/ch_convergencetemporal_SecondOrder1_voronoi_p4}
            \end{center}
        }
        \label{tab: voronoi grid result}
    \end{table}
}{
    \begin{table}
        \addtolength{\tabcolsep}{-0.5pt}
        {\footnotesize
            \captionsetup{position=top}
            \caption{
                Test 1: $L^2, H^1,$ and $H^2$ errors and convergence rates for the convergence test on a Voronoi polygonal grid.
                }
            % \begin{center}
                \input{Results/TablesRevised/ch_convergencetemporal_FE-BE_voronoi_p2}
                \\
                \input{Results/TablesRevised/ch_convergencetemporal_SecondOrder1_voronoi_p2}
                \\
                \input{Results/TablesRevised/ch_convergencetemporal_SecondOrder1_voronoi_p4}
            % \end{center}
        }
        \label{tab: voronoi grid result}
    \end{table}
}

==> Sections/Results.tex <==
\section{Numerical Results}\label{sec: numerical testing}
In this section we present a fully discrete scheme and investigate its behaviour numerically.
The fully discrete scheme couples the VEM spatial discretization with a Runge-Kutta (RK) scheme, which combines a convex splitting (CS) method with a multi-stage additive RK method. 
\corrections{Since we present a higher order spatial discretization we couple the VEM discretization with a higher order time stepping method.}
We use a nonlinear convex splitting of the energy $E(u)$, defined in \eqref{eqn: energy functional}, see e.g. \cite{elliott1993global,eyre1998unconditionally1,lee2020stability,shin2017unconditionally}, where we split the energy into a contractive and expansive part as follows
\begin{align*}
    E(u) = E_c(u) - E_e(u) = \int_{\Omega} \left( \frac{u^4}{4} + \frac{1}{4} + \frac{\eps^2}{2} |\nabla u |^2 \right) \, \dx - \int_{\Omega} \frac{u^2}{2} \, \dx,
\end{align*}
where $E_c(u)$ is treated implicitly \corrections{while} $E_e(u)$ is treated explicitly. 
It is straightforward to show that $E_c(u)$ and $E_e(u)$ are both convex.
\ifthenelse{\boolean{thesis}}{
    We denote two RK methods using standard Butcher notation
    \begin{align}\label{eqn: Butcher table}
        \begin{array}{c|c}
            c & A
            \\
            \hline
            & b^T      
        \end{array}
        =
        \begin{array}{c|ccc}
            c_1 & a_{11} & \cdots & a_{1s} 
            \\   
            \vdots & \vdots & \ddots & \vdots
            \\
            c_s & a_{s1} & \cdots & a_{ss}
            \\
            \hline
            & b_{1} & \cdots & b_{s}   
        \end{array}
        ,
        \quad 
        \begin{array}{c|c}
            \hat c & \hat A
            \\
            \hline
            & \hat b^T        
        \end{array}
        =
        \begin{array}{c|ccc}
            \hat c_1 & \hat a_{11} & \cdots & \hat a_{1s} 
            \\   
            \vdots & \vdots & \ddots & \vdots
            \\
            \hat c_s & \hat a_{s1} & \cdots & \hat a_{ss}
            \\
            \hline
            & \hat b_{1} & \cdots & \hat b_{s}   
        \end{array}
    \end{align}
    for $A, \hat A \in \R^{s \times s}$, $b,\hat b \in \R^s$ and the coefficients $c, \hat c \in \R^s$ are given by $c=A1, \hat c = \hat A1$. 
}{}

\begin{definition}[Fully discrete scheme]
    We split $[0,T]$ into uniform subintervals, \corrections{each of length $\tau=T/\hat N$} and \corrections{discretize} the solution at time $t_n$, \corrections{${n=0,\dots,\hat N}$,} \corrections{as} $u^{n}_{h \tau} = u_h(\cdot,t_n) \in \vemSpace$. We first split the semilinear form $r_h$ according to the convex splitting above,
    recalling that ${\phi^{\prime} (w) = 3w^2 - 1}$, this is given by
    \begin{align*}
        r_{h,c}  ( u_{h \tau}^n ; v_h, w_h ) &-  r_{h,e} ( u_{h \tau}^n ; v_h, w_h )
        \\
        &
        =
        \sum_{K \in \mesh} \int_K 3 ( u_{h \tau}^n)^2 \gradProj v_h \cdot \gradProj w_h \, \dx
        -
        \sum_{K \in \mesh} \int_K \gradProj v_h \cdot \gradProj w_h \, \dx
    \end{align*}
    for $u_{h \tau}^n, v_h, w_h \in \vemSpace$. 
    Our fully discrete scheme is therefore \corrections{as follows: given $u^0_{h \tau} = u_{h,0} \in \vemSpace$, for $n=0,\dots,\hat N-1,$ find $u_{h \tau}^n \in \vemSpace$ such that}   
    \begin{align*}
        m_h ( u^{n+1}_{h \tau} - u^n_{h \tau} , v_h )
        + \tau \sum_{i=1}^s &\bigg(
        b_i \left( \eps^2 a_h ( U^i , v_h) + r_{h,c} ( \Pi^h_0 U^i ; U^i, v_h) \right) 
        \\
        &- 
        \hat b_i r_{h,e} ( \Pi^h_0 U^i ; U^i, v_h) \bigg) = 0
    \end{align*}
    % for all $v_h \in \vemSpace$,
    where the $i$-th stage is defined by
    \begin{align*}
        m_h ( U^i - u^n_{h\tau},v_h ) + \tau \sum_{j=1}^s &\bigg(
        a_{ij} \left( \eps^2 a_h ( U^j , v_h) + r_{h,c} ( \Pi^h_0 U^j ; U^j, v_h) \right)
        \\ 
        &- \hat a_{ij} r_{h,e} ( \Pi^h_0 U^j ; U^j, v_h) \bigg) = 0  
    \end{align*}
    for all $v_h \in \vemSpace$, for $i=1,\dots,s$.
    The coefficients are defined using standard Butcher notation for RK methods and satisfy $A, \hat A \in \R^{s \times s}$, $b,\hat b \in \R^s$. 
    % and the $c, \hat c \in \R^s$ are given by $c=A1, \hat c = \hat A1$. 
\end{definition}

The first scheme we use is the simple first order CS ``Forward-Backward Euler" method (CSRK-1) \cite{shin2017unconditionally}, with the standard Butcher notation
\begin{align}\label{eqn: IMEX1 Butcher tables}
    \begin{array}{c|c}
        c & A 
        \\
        \hline
        & b^T        
    \end{array}
    =
    \begin{array}{c|cc}
        0 & 0 & 0 
        \\
        1 & 0 & 1 
        \\   
        \hline
         & 0 & 1   
    \end{array}
    ,
    \quad 
    \begin{array}{c|c}
        \hat c & \hat A 
        \\
        \hline
        & \hat b^T        
    \end{array}
    =
    \begin{array}{c|cc}
        0 & 0 & 0 
        \\
        1 & 1 & 0 
        \\   
        \hline
         & 1 & 0   
    \end{array}
    .
\end{align}
The other method we consider is the second order CS Runge-Kutta method (CSRK-2) presented in \cite{lee2020stability}, rewritten in Butcher notation as
\begin{align}\label{eqn: IMEX2 Butcher tables}
    \begin{array}{c|c}
        c & A 
        \\
        \hline
        & b^T        
    \end{array}
    =
    \begin{array}{c|cccc}
        0 & 0 & 0 & 0 & 0\\
        1 & 0 & 1 & 0 & 0\\
        \frac{3}{2} & 0 & \half & 1 & 0\\
        1 & 0 & 1 & -1 & 1 \\
        \hline
        & 0
        & 1 
        & 
        -1
        &
        1
    \end{array}
    ,
    \qquad
    \begin{array}{c|c}
        \hat c & \hat A 
        \\
        \hline
        & \hat b^T        
    \end{array}
    =
    \begin{array}{c|cccc}
        0 & 0 & 0 & 0 & 0\\
        1 & 1 & 0 & 0 & 0\\
        \frac{3}{2} & \half & 1 & 0 & 0\\
        1 & 1 & -1 & 1 & 0\\
        \hline
        & 1 
        & 
        -1
        &
        1
        &
        0
    \end{array}
    .
\end{align}
The schemes defined in both \eqref{eqn: IMEX1 Butcher tables} and \eqref{eqn: IMEX2 Butcher tables} are shown to be energy stable for the semidiscrete (continuous-in-space) schemes \cite{lee2020stability,shin2017unconditionally}. 
We \emph{numerically} investigate the energy decay property of our proposed fully discrete scheme in Test 3 in Section~\ref{sec: evo cross}.

\corrections{We point out that the lowest order ($\polOrder=2$) nonconforming VEM on triangles is identical to the Morley nonconforming finite element and so, with the exception of Test 1 in Section~\ref{subsec: test 1}, we only investigate the behaviour of the higher order $\polOrder=4$ VEM since the other case has been studied extensively in the literature.}

The code we use to carry out the simulations is based on the Distributed and Unified Numerics Environment (\textsc{Dune}) software framework \cite{dunegridpaperII} and has been implemented within the \textsc{Dune-Fem} module \cite{dedner2010generic}. 
\textsc{Dune} is open source software implemented in \texttt{C++}, but since a user has access to a Python frontend \cite{dedner_dune_2018}, they can easily perform numerical experiments by describing mathematical models using the domain specific form language UFL \cite{alnaes_unified_2012}. 
Tutorials including some VEM examples can be found in \cite{dedner2020python} \corrections{while further implementation details can be found in \cite{dedner2022framework}}.

\ifthenelse{\boolean{thesis}}{
% subsection with VEM convergence test, don't include here but submit in thesis chapter. 
\subsection{Test 1: VEM convergence}
For this first experiment we investigate convergence to an exact solution to verify convergence of our VEM discretization applied to the Cahn-Hilliard equation. We set the forcing $f$ so that the exact solution is given by 
\begin{align*}
    u(x,y,t) = \sin(2\pi t)\cos(2\pi x)\cos(2\pi y). 
\end{align*}
In this test we use a small time step, namely $\tau=10^{-5}$ and fix $\eps = 1/10$. We run the convergence test on both a structured simplex grid and a Voronoi grid for discretizing the unit square. The $L^2, H^1,$ and $H^2$ errors are computed at every time step and we present the maximum errors in each case.

We investigate the convergence for polynomial orders $\polOrder=2$ and for the first order Forward-Backward Euler (CSRK-1) \eqref{eqn: IMEX1 Butcher tables} time stepping method. 

The results detailed in Tables \ref{tab: ch_convergencespatial_FE-BE_criss_p2} and \ref{tab: ch_convergencespatial_FE-BE_voronoi_p2} show the errors and experimental orders of convergence (eocs) from Test 1, and are consistent with the result from Theorem \ref{thm: L2 convergence}. 

% \input{Results/TablesRevised/ch_convergencespatial_FE-BE_criss_p2}
% \input{Results/TablesRevised/ch_convergencespatial_FE-BE_voronoi_p2.tex}


}
{}

% \red{Make a remark that we will focus on CSRK-2 and $l=4$ except for Test 1 and why}
% -----------------------------------------------------------------------------------
% -- Convergence test
% -----------------------------------------------------------------------------------

\subsection{Test 1: \corrections{Convergence to an exact solution}}\label{subsec: test 1}
The first numerical experiment we consider is a non-physical test to recover the order of convergence presented in Theorem~\ref{thm: L2 convergence} 
\corrections{as we investigate convergence} to a \corrections{known} exact solution.
In this test we reduce $\tau$ alongside $h$, starting with $\tau = 10^{-2}$. We fix $\eps = 1/10$ for these experiments and run them on both the structured simplex ``criss'' grid consisting of half square triangles and a sequence of Voronoi grids discretizing the unit square $\Omega = (0,1)^2$. 
The Voronoi grids are randomly seeded and smoothed using Lloyd's algorithm.
The $L^2, H^1,$ and $H^2$ errors are computed at every time step and we present the maximum errors in each case.
We set the forcing $f$ so that the exact solution is given by 
\begin{align*}
    u(x,y,t) = \sin(2\pi t)\cos(2\pi x)\cos(2\pi y). 
\end{align*}
This is a modification of the test considered in e.g. \cite{antonietti_$c^1$_2016,chave2016hybrid}
where we have changed the exact solution to be nonlinear in $t$.   

We investigate the convergence for polynomial orders $\polOrder=2,4$ for the CSRK-1 \eqref{eqn: IMEX1 Butcher tables} and CSRK-2 \eqref{eqn: IMEX2 Butcher tables} time stepping methods. 
\corrections{For the sake of brevity we don't show results for $\polOrder=3$ but note that they are in line with expectations.}   
The results on the simplex and Voronoi polygonal grids are shown in Tables~\ref{tab: ch_convergencetemporal_FE-BE_criss_p2}-\ref{tab: ch_convergencetemporal_SecondOrder1_criss_p4} and Tables~\ref{tab: ch_convergencetemporal_FE-BE_voronoi_p2}-\ref{tab: ch_convergencetemporal_SecondOrder1_voronoi_p4}, respectively.

The results from this convergence test are in line with expectations. Since the CSRK-1 method is first order accurate in time and the CSRK-2 method is second order accurate, when combining one of these methods with the order $\polOrder$ VEM method, we should expect to see $L^2$ convergence rates of order $\min\{ \polOrder,m \}$ where $m \in \{1,2 \}$ is the order from the CSRK-$m$ method. 
To see the optimal $L^2$ convergence $O(h^{\polOrder})$ (Theorem \ref{thm: L2 convergence}), we look at the $\polOrder=2$ VEM method coupled with the CSRK-2 time stepping. 
These results are shown in Tables~\ref{tab: ch_convergencetemporal_SecondOrder1_criss_p2} and \ref{tab: ch_convergencetemporal_SecondOrder1_voronoi_p2}.

Note that the convergence rates in the $H^1$ and $H^2$ norms are also what we would expect to see if we extended Theorem \ref{thm: L2 convergence} to include convergence results in both $H^1$ and $H^2$ norms according to classic FE theory. 
\corrections{For example, the rate for the $H^2$ error with $\polOrder=2$ is equal to $1$ while the higher order is clearly visible in the $\polOrder=4$, CSRK-2 results (Tables~\ref{tab: ch_convergencetemporal_SecondOrder1_criss_p4} and \ref{tab: ch_convergencetemporal_SecondOrder1_voronoi_p4}).}

% \begin{table}\label{tab: test 1 simplex grid result}
    % \subcaption{Test 1: $L^2, H^1,$ and $H^2$ errors and convergence rates for the convergence test on a structured simplex grid.}
    \input{Results/TablesRevised/ch_convergencetemporal_FE-BE_criss_p2}
    \input{Results/TablesRevised/ch_convergencetemporal_SecondOrder1_criss_p2}
    \input{Results/TablesRevised/ch_convergencetemporal_SecondOrder1_criss_p4}
% \end{table}         

% \begin{table}\label{tab: test 1 voronoi grid result}
    % \caption{Test 1: $L^2, H^1,$ and $H^2$ errors and convergence rates for the convergence test on a Voronoi polygonal grid.}
    \input{Results/TablesRevised/ch_convergencetemporal_FE-BE_voronoi_p2}
    \input{Results/TablesRevised/ch_convergencetemporal_SecondOrder1_voronoi_p2}
    \input{Results/TablesRevised/ch_convergencetemporal_SecondOrder1_voronoi_p4}
% \end{table}

% -----------------------------------------------------------------------------------
% -- Two bubbles
% -----------------------------------------------------------------------------------
\input{Results/FiguresRevised/twoellipse}


\subsection{Test 2: Two interacting bubbles}\label{subsec: test 2}
\corrections{This test is taken from} \cite{feng2008posteriori,wu2020analysis} \corrections{and is dedicated to the evolution of two ellipses.}
A similar test is investigated in \cite{liu2020fully}.
\corrections{In particular, we take initial data as follows}
\begin{align*}
    u_0(x,y) = {\rm tanh} \left( ((x-0.3)^2 + y^2 - 0.25^2 ) / \eps \right){\rm tanh} \left( ((x+0.3)^2+y^2-0.3^2 )/ \eps\right) 
\end{align*}
where ${\rm tanh}(t) = (e^t - e^{-t})/(e^t+e^{-t})$. 
We monitor the evolution of two ellipses on the domain $\Omega=(-1,1)^2$ and fix $\polOrder=4$, $\eps=3/100$ \corrections{for this experiment}.
\corrections{We use the CSRK-2 \eqref{eqn: IMEX2 Butcher tables} time stepping method with $\tau=10^{-3}$. 
We show results on the $25 \times 25$ Voronoi mesh.
The screenshots of the numerical interface at 6 different fixed time frames is shown in Figure~\ref{fig: zero level sets}.
Here we see that the initial ellipses evolve and
coalesce over time to one ellipse. Note that the observed behaviour and evolution of
the interface is in line with the results displayed in \cite{wu2020analysis} for the Morley element.}

\FloatBarrier


% -----------------------------------------------------------------------------------
% -- Cross evolution
% -----------------------------------------------------------------------------------
\subsection{Test 3: Evolution of a cross}\label{sec: evo cross}
As considered in e.g. \cite{antonietti_$c^1$_2016,chave2016hybrid,liu2020fully}, for this experiment we monitor the evolution of initial data relating to a cross-shaped interface between phases. The initial data is described as follows.
\begin{align*}
    u_0(x,y) = \begin{cases}
        0.95 \quad &\text{ if }\quad  |(y-\half) - \frac{2}{5}(x-\half)| + | \frac{2}{5}(x-\half) + (y-\half) | < \frac{1}{5},
        \\
        0.95 \quad &\text{ if }\quad  |(x-\half) - \frac{2}{5}(y-\half)| + | \frac{2}{5}(y-\half) + (x-\half) | < \frac{1}{5},
        \\
        -0.95 \quad &\text{ otherwise.}
    \end{cases}
\end{align*}

We carry out this experiment on the unit square using \corrections{the same two mesh types as in Test 1 (as described in Section~\ref{subsec: test 1}) for three different grid sizes.
The grid data for these choices is detailed in Table~\ref{tab: grid size data} alongside the total number of dofs for each of these grid sizes.}
We also take multiple values for the interface parameter: ${\eps = 1/100, 1/50,}$ and $1/25$ and investigate the behaviour of the method for each \emph{fixed} value of epsilon. 
We also fix $\tau = 10^{-3}$, use the CSRK-2 time stepping method \eqref{eqn: IMEX2 Butcher tables} for these simulations and run the test to time $T=0.8$. 

\input{Results/TablesRevised/grid_data}

\corrections{We only show the evolution of the method for this test on the $25 \times 25$ grids for two of the values of interface parameter $\eps=1/100$ (Figure~\ref{fig: evolutionScreenshots criss}) and $\eps=1/25$ (Figure~\ref{fig: evolutionScreenshots voronoi}) at three different fixed time frames.
We overlay the grids in the first images in Figures~\ref{fig: evolutionScreenshots criss} and \ref{fig: evolutionScreenshots voronoi}.}

\corrections{Figures~\ref{fig: end times for Test 2 screenshots simplex} and \ref{fig: end times for Test 2 screenshots voronoi} show the evolution at the end time frame ($T=0.8$) for $\eps=1/100$ and $\eps=1/25$, respectively for both the simplex criss mesh and Voronoi mesh.
We show the grids overlaid in the first figure, Figure~\ref{fig: end times for Test 2 screenshots simplex}.
Each figure contains the end time frame for all grid sizes from left to right $15 \times 15, 25 \times 25$, and $45 \times 45$.
We can see from Figures~\ref{fig: end times for Test 2 screenshots simplex} and \ref{fig: end times for Test 2 screenshots voronoi} that in all cases the initial data evolves to a circular interface even for the coarse $15 \times 15$ grid. 
Again, for the sake of brevity, we do not show the end evolution for $\eps=1/50$.}

\corrections{The energy decay for this problem is shown in Figure \ref{fig: energy plots}.
At each time step we compute the energy $E(u_h)$ \eqref{eqn: energy functional} of the discrete solution $u_h$.
As expected, the energy decreases in nearly all cases.
There is a slight increase in the left figure of Figure~\ref{fig: energy plots eps=1/100} which corresponds to the interface parameter $\eps=1/100$ on the coarse $15 \times 15$ criss grid, indicating that the interface is unresolved even with the higher order scheme on this grid.
We also see in Figures~\ref{fig: end times for Test 2 screenshots simplex} and \ref{fig: end times for Test 2 screenshots voronoi} a slightly larger circular interface on the coarsest grids.} 

% \FloatBarrier
% -----------------------------------------------------------------------------------
% -- Spinodal decomposition
% -----------------------------------------------------------------------------------

\subsection{Test 4: Spinodal decomposition}
For this experiment we turn our attention to the spinodal decomposition of a binary mixture. 
\corrections{As} in \cite{antonietti_$c^1$_2016,chave2016hybrid}, to model this phenomenon we choose the initial data $u_0$ to be a random perturbation between $-1$ and $1$ located in a circle of diameter $0.3$ in the centre of the domain and $0$ elsewhere. 
We take the interface parameter to be $\eps=1/100$, with time step $\tau = 10^{-2}$, and we use the CSRK-2 time stepping method \eqref{eqn: IMEX2 Butcher tables}. 
Snapshots of the results on both the structured simplex
grid and the Voronoi polygonal mesh are shown in Figure~\ref{fig: Test 3 results for p=4 on both grids}.
% We only present the results from this test for $\polOrder=4$ but note that the results for lower orders ($\polOrder=2,3$) \corrections{are} analogous.
Note that the random initial conditions used for the two grids are different and result in the difference in the end configurations seen in Figure \ref{fig: Test 3 results for p=4 on both grids}.

\input{Results/FiguresRevised/evolutionNew}
\input{Results/FiguresRevised/endScreenshots}
\input{Results/FiguresRevised/Random/evolutionScreenshots}
\FloatBarrier
\input{Results/Data/energyPlots}




\FloatBarrier

\subsection{Comparison with conforming VEM}
\jsccorrections{In this section we briefly investigate numerically the behaviour of the $C^1$-conforming virtual element method, see e.g. \cite{antonietti_conforming_2018,brezzi_virtual_2013}.
A full set of numerical experiments for the lowest order $C^1$ method can be found in \cite{antonietti_$c^1$_2016}.
However, note that the treatment of the nonlinearity in \cite{antonietti_$c^1$_2016} differs from the approach taken in this paper.
Whilst the $C^1$ VEM has the advantage of being conforming in $H^2$, the implementation of the nonconforming VEM presented in this paper is simpler.
For example, the treatment of boundary conditions is more complex for the conforming space due to the tangential derivative degrees of freedom at the vertices.
The lowest order $C^1$ VEM ($\polOrder=2$) has only 3 degrees of freedom per vertex so on structured triangular grids (such as the ``criss'' grid considered in this section) it will generally have fewer dofs than the nonconforming space; however, this is not the case on other polygonal grids such as either structured quadrilateral grids or Voronoi grids.
Additionally, due to only having 9 dofs on triangles, extra care is required when implementing the value projection for the $C^1$-conforming VEM.
%  as this space does not fit straightforwardly into the framework introduced in \cite{dedner2022framework}. 
Further discussion on this as well as implementation details for both spaces can be found in \cite{dedner2022framework}. 
}

\jsccorrections{
    In this work, we have focused on developing higher order extensions of Morley which is often the only space available in finite element packages for solving fourth-order problems.
    Consequently, the tools and infrastructure necessary to implement the higher order nonconforming VEMs in this paper is likely to be more readily available.
    Importantly, for all grid resolutions considered in the tests so far, the advantage of using the higher order method is apparent.
    On top of this, we see in the subsequent comparison that both the higher order conforming and nonconforming VEM produce identical results.}

\jsccorrections{
We now turn our attention to repeating some of the tests already presented but with the $C^1$-conforming VEM.
Firstly, we repeat the non-physical test, Test 1 from section~\ref{subsec: test 1}.
We select the exact same parameters as in section~\ref{subsec: test 1} and the results on the structured simplex ``criss'' grid with the CSRK-2 \eqref{eqn: IMEX2 Butcher tables} time stepping method are shown in Figure~\ref{fig: test1 plots} for polynomial orders $\polOrder=2,3,4$.
We plot the $H^2$-error in the left figure for both the $C^1$-conforming and the nonconforming spaces and the order of convergence is shown in the right figure.
Since we use a second order time stepping method, the eocs for $\polOrder=3,4$ are the same.
For the lowest order spaces ($\polOrder=2$), we see that the $C^1$-conforming VEM outperforms the nonconforming space however, the results for $\polOrder=3,4$ are indistinguishable.
We point out that the same is true when looking at grid size $h$ vs error as well as dofs vs error.}

\jsccorrections{
Secondly, we investigate Test 2 with the $C^1$-conforming space. 
We use the exact same parameters as detailed in section~\ref{subsec: test 2} and the results are shown in Figure~\ref{fig: zero level sets C1conf version}.
As for the nonconforming space, the initial ellipses evolve and coalesce over time to one ellipse.
Despite the lowest order $C^1$-conforming VEM producing better errors for the non-physical test of Test 1, we point out that the results from this test are essentially identical to those shown in Figure~\ref{fig: zero level sets}.}



\input{Results/Data/test1.tex}
\input{Results/C1conf/TwoEllipse/C1conf_twoellipse.tex}
\FloatBarrier

==> Setup/abstract.tex <==
\begin{abstract}
    In this paper we develop a fully nonconforming virtual element method (VEM) of arbitrary approximation order for the two dimensional Cahn-Hilliard equation. 
    We carry out the error analysis for the continuous-in-time scheme and verify the theoretical convergence result via numerical experiments. 
    We present a fully discrete scheme which uses a convex splitting Runge-Kutta method to discretize in the temporal variable alongside the virtual element spatial discretization. 
\end{abstract} 

\begin{keywords}
    virtual element method, 
    Cahn-Hilliard equation, nonlinear, fourth-order problems, nonconforming, DUNE.
\end{keywords}

\begin{AMS}
    65M12, 65M60
\end{AMS}

==> Setup/preamble.tex <==
\usepackage{mathptmx}
\usepackage{graphicx}
% \usepackage{epstopdf}
\usepackage{amsmath}
\usepackage{amssymb}
% \usepackage{enumerate}
% \usepackage{enumitem}
\usepackage{mathtools}
% \usepackage[nodayofweek]{datetime} 
% \usepackage[framemethod=tikz]{mdframed}
\usepackage{tikz}
% \graphicspath{{Fig/}}
% \graphicspath{{images/}}
% \usepackage{listings}
% \usepackage[draft]{todonotes} 
\usepackage{comment}
% \usepackage{authblk}
\usepackage{booktabs}
% \usepackage[font=small]{caption}
% \usepackage[font=small]{subcaption}
% \usepackage{float}
% \usepackage{multirow}
\usepackage{placeins} % for floatbarrier
\usepackage{ifthen}
\usepackage{pgfplots}
% \usepackage{siunitx}
\usepackage{subfig}
\usepackage{array}
\usepackage{doi}
% \usepackage{capt-of}
% \pgfplotsset{every tick label/.append style={font=\tiny}}
\pgfplotsset{compat=1.18}
%------------------------------------------------------------
% \pgfplotsset{compat=newest} % Allows to place the legend below plot
% \usepgfplotslibrary{units} % Allows to enter the units nicely
% \sisetup{
%   round-mode          = places,
%   round-precision     = 2,
% }
% \usetikzlibrary{external}
% \tikzexternalize


%------------------------------------------------------------

% \numberwithin{equation}{section} % number equations within sections 
\spdefaulttheorem{assumption}{Assumption}{\bf}{\it}

\allowdisplaybreaks % allow equations to break over leaf

